Towards Coinductive Theory Exploration in Horn Clause Logic: Position Paper

Coinduction occurs in two guises in Horn clause logic: in proofs of self-referencing properties and relations, and in proofs involving construction of (possibly irregular) infinite data. Both instances of coinductive reasoning appeared in the literature before, but a systematic analysis of these two kinds of proofs and of their relation was lacking. We propose a general proof-theoretic framework for handling both kinds of coinduction arising in Horn clause logic. To this aim, we propose a coinductive extension of Miller et al's framework of uniform proofs and prove its soundness relative to coinductive models of Horn clause logic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{27}
\providecommand{\publicationstatus}{T. Kahsai and G. Vidal (Eds.): 5th Workshop on\\ Horn Clauses for Verification and Synthesis 2018 (HCVS'18).\\
EPTCS 278, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.278.5}{10.4204/EPTCS.278.5}}
\pdfoutput=1

